Pros & Cons of Model-based Bandwidth Control for Client-assisted Content Delivery

A key challenge in \cacd\ is determining how to allocate limited server bandwidth across a large number of files being concurrently served so as to optimize global performance and cost objectives. In this paper, we present a comprehensive experimental evaluation of strategies to control server bandwidth allocation. As part of this effort, we introduce a new {\em model-based} control approach that relies on an accurate yet concise "cheat sheet" based on a priori offline measurement to predict swarm performance as a function of the server bandwidth and other swarm parameters. Our evaluation using a prototype system, \cs, instantiating static, dynamic, and model-based controllers shows that static and dynamic controllers can both be suboptimal due to different reasons. In comparison, a model-based approach consistently outperforms both static and dynamic approaches provided it has access to detailed measurements in the regime of interest. Nevertheless, the broad applicability of a model-based approach may be limited in practice because of the overhead of developing and maintaining a comprehensive measurement-based model of swarm performance in each regime of interest.

==> background.tex <==
%\section{Background and goals}


\section{Server capacity control}
\label{sec:bg}

%\subsection{Server capacity control}

\subsection{Background and goals}
We assume that the reader is familiar with peer-to-peer swarming and BitTorrent \cite{bittorrent} in particular. A brief introduction may be obtained in \cite{Kurose-Ross} or the background sections of recent papers on swarming (e.g., \cite{bittyrant, BTauction}).

Managed swarming seeks to get achieve the best of client-server file distribution and peer-to-peer swarming, namely, the predictable performance and ease of management of the former and the bandwidth cost savings of the latter. In addition to a tracker for each file, we assume the presence of an always online seed (referred to as the {\em server} or {\em publisher}). Users interested in downloading the file (or {\em peers}) are assumed to be non-altruistic, i.e., they leave as soon as they complete their download. The server seeks to opportunistically leverage peer-to-peer bandwidth when possible and, if necessary, uses its own bandwidth to distribute the file.

%This paper focuses on the problem of server (seeder) capacity control for BitTorrent. 

\subsubsection{Goals}
Our goal is to design and implement a system to allocate server bandwidth across multiple managed swarms so as to optimize system-wide performance or cost objectives. Although this problem has received some research attention in recent times, our design requirements listed below compel us to revisit this problem.
\begin{enumerate}
\item {\em Protocol-compatibility}: The server capacity allocation system should be compatible with the widely used BitTorrent wireline protocol. Protocol compatibility enables the system to interoperate with the huge base of BitTorrent users.
\item {\em Unmodified clients}: The system should work effectively with existing BitTorrent clients and not require users to download new client software.
\item {\em Flexibility}: The system should be able to support a variety of  optimization objectives to improve aggregate performance or cost  metrics of interest to administrators. 
\item {\em Simplicity}: The system should require minimal information from peers in order to make its bandwidth allocation decisions.
\end{enumerate}

The above design requirements distinguish our work from recently developed systems \cite{antfarm,vformation} with similar goals. In particular, both AntFarm and V-Formation propose new protocols that are incompatible with BitTorrent, and require server- as well as client-side changes. These changes are required to obtain a fine-grained block-level information about a peer's uploads to other peers both for monitoring performance as well as selfish behavior. A more detailed comparison of \cs\ and AntFarm is discussed in Section \ref{sec:related}.


%In particular, we seek a solution which is protocol compatible, requires minimal information from peers, and works for a variety of objectives. The merit of protocol-compatible solution lie in leveraging a multitude of BitTorrent client implementations and a huge base of BitTorrent users. We insist on requiring minimal per-peer information to keep the system simple. The ability to support multiple objectives for a set of swarms such as maximizing the minimum download rate of a swarm, maximizing the average download rate for peers  allows the content publisher the freedom to choose one. 


%The above requirements distinguish our problem from prior systems such as AntFarm and V-Formation. Both AntFarm and V-Formation propose a new protocol which is incompatible with BitTorrent, require  block-level information about each peer's uploads to other peers, and are designed to optimize the same objective: aggregate bandwidth of a set of swarms.

\eat {

The server bandwidth allocation to a swarm depends on its \emph{response curve} \cite{antfarm}, i.e., the curve predicting the chosen performance metric for a swarm (e.g. average download rate)  as a function of seeder bandwidth. The response curve for a swarm depends on the performance metric chosen and the way a  BitTorrent swarm is modeled.

% our BitTorrent model
A key feature of our model of a BitTorrent swarm is that we model peers joining the swarm as a poisson process. Each peer contributes to the swarm until it finishes its file download. Thereafter, it immediately departs from the swarm. Due to arrival and departure of peers, the number of peers in the swarm at any point does not remain constant. Even the average number of peers is not fixed, but depends on the average arrival rate as well as the download time of each peer.\footnote[1]{The average number of peers follows from Little's law \cite{Little's Law}, which is $N = \lambda T$, $N$ = average number of peers,  $\lambda$ is the average arrival rate, $T$ is the average duration of peers in the system.} Our performance metric for a swarm is the average download time for a peer, which we believe is reasonable for BitTorrent since it is used primarily to download large files. 

% Different between our model and flash-crowd model
We distinguish our model from an alternate model presented in \cite{antfarm} which models a flash-crowd scenario. In the flash-crowd model, a swarm has a fixed number of peers, $N$, which join the swarm at the same time and start downloading a very large file. Lets assume that all peers have same upload bandwidth. If the seeder uploads at a rate which is less than the upload bandwidth at each peer, each block is uploaded only once by the seeder and is distributed among all peers through peer-to-peer exchanges. Thus, download rate of each peer is equal to the seeder upload rate and is independent of the number of peers in the swarm. 

There are two important differences between the two models. First, unlike the flash-crowd model, the number of peers in a swarm in our model is a time varying function of the peer arrival rate and the download time for each peer.  Second, the response curve of average download rate vs. the seeder bandwidth  in a flash crowd model is linear as explained above.  The empirically measured response curves for our model show a concave behavior and  concavity increases with an increase in the arrival rate of peers.
}


\subsection{Controller strategies classification}

% static

We classify the approaches for server capacity control into three categories: (1) static, (2) dynamic, and (3) model-based. A static controller partitions bandwidth statically across competing swarms.

%We define few baseline controller strategies for comparison, which we term static controllers.  An example of a static controller is \eqsplit, that is this controller splits the seeder bandwidth equally among all the swarms. 

% dynamic:
A dynamic controller periodically takes measurements of swarm performance and adjusts seeder bandwidth in response to it. An example of dynamic controller is the system  AntFarm \cite{antfarm}, which uses measurements of download rate at each peer in order to calculate the bandwidth allocation to each swarm. A dynamic controller needs to be designed based on the objective function. For example, the bandwidth allocation to swarms computed by AntFarm  maximizes the aggregate download rate of a set of swarms, but it may perform poorly for another objective function such as maximizing the {\em mean} download rate of peers, or maximizing the worst-case performance across multiple swarms.


A third-type of controller, which we call a model-based controller, uses a model to predict the performance of a swarm. This model predicts the performance of a swarm as a function of the server bandwidth allocated to it and other parameters of the swarm such as the peer arrival rate, the upload capacity distribution across peers, and the size of the file. If such a model can be developed, a model-based controller can directly ``jump'' to the optimal bandwidth allocation by solving the corresponding optimization problem ``on paper'' as opposed to searching for the optimal allocation in situ like the dynamic control approach described above. A key focus of our work is to determine the feasibility of developing such a model and comparing the performance of a model-based approach to a dynamic control approach.

We focus on three different performance objectives in this paper: (1) \maxavg, that seeks to maximize the average download time across all peers across all swarms; (2) \maxmin, that seeks to  minimize the average download time of the swarm with the highest average download time; and (3) \mincost, that seeks to minimize the server bandwidth consumed so as to achieve a set of target download times specified for the swarms while minimizing the overall server bandwidth consumed.

% The role of the controller is to calculate a bandwidth allocation which optimizes a given objective. If a model is given and the swarm parameters are known, a bandwidth allocation which optimizes a given objective function, can be calculated in an offline manner using paper calculations, or in the worst case through exhaustively searching through possible seeder bandwidths values to maximize the objective function. The first challenge of a model based approach are first in coming up with a model based on easily estimable parameters. Even so a model based approach is  likely to suffer from modeling errors, in which case a well-designed dynamic controller for that objective can perform  better than a model-based controller. 

%The goal of this work is to  and and a model 
%Our wor
%Our central motivation behind this work is to design both onlnie 
%Any optimization can be computed for a set of swarms. 
%
%While a dynamic controller requires measurements of swarm performance, a model-based 
%
%Such a controller faces the challenge of estimating swarm parameters
%Such a 
%
%can predict the performance of the swarm 
%does not take into account the average download rate of the swarm. 
%
%
%A dynamic controller needs to be designed keeping the objective into account. A controller which optimizes the \maxavg\ objective may look 
%
%Such a controller needs to be designed to optimize an objective function. 





% model based
% (1) online control : relies on active measurement of swarm performance and adjusts server bandwidth in response to changes in measured performance of the swarm. 
%
%
%Antfarm takes long time to build response curves. V-Formation uses light weight probes but relies on block level measurements across the swarm. 
%
%
%We define offline control as a technique which requires minimal information about a swarm, specifically no active measurements in order to predict the performance of a swarm. The above definition of offline control leads us to two tasks:
%
%(1) Determine the minimal set of parameters which most significantly determine the performance of a swarm.
%
%(2) Develop a model which can predict the response curve of a swarm given the set of minimal swarm parameters.
%
%As we saw in the above example using figure 1. If response curves for a swarm can be predicted in an offline manner,this automatically yields an offline server capacity control technique. 
%
%Two more questions:
%
%(1) what if response curve changes
%
%(2) altruistic peers, multiple swarm membership, 

%b. Is it necessary to rely on block level measurements for each swarm or a simpler coarse grained measurement of aggregate swarm characteristics sufficient for offline control ?

